Introduction to Toric Geometry

These notes are based on a series of lectures given by the author at the Max Planck Institute for Mathematics in the Sciences in Leipzig. Addressed topics include affine and projective toric varieties, abstract normal toric varieties from fans, divisors on toric varieties and Cox's construction of a toric variety as a GIT quotient. We emphasize the role of toric varieties in solving systems of polynomial equations and provide many computational examples using the Julia package Oscar.jl.

==> path.tex <==
\catcode`:=\active
\def:{\par}

\parindent0pt\tt

\input|"echo $PATH"

\bigskip

Is there pygmentize?

\input|"which pygmentize"

\bye
